Intersection Types and Counting

We present a new approach to the following meta-problem: given a quantitative property of trees, design a type system such that the desired property for the tree generated by an infinitary ground lambda-term corresponds to some property of a derivation of a type for this lambda-term, in this type system. Our approach is presented in the particular case of the language finiteness problem for nondeterministic higher-order recursion schemes (HORSes): given a nondeterministic HORS, decide whether the set of all finite trees generated by this HORS is finite. We give a type system such that the HORS can generate a tree of an arbitrarily large finite size if and only if in the type system we can obtain derivations that are arbitrarily large, in an appropriate sense; the latter condition can be easily decided.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{N. Kobayashi (Ed.): Eighth Workshop\\
on Intersection Types and Related Systems (ITRS 2016).\\
EPTCS 242, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.242.6}{10.4204/EPTCS.242.6}}

